Probability bound analysis: A novel approach for quantifying parameter uncertainty in decision-analytic modeling and cost-effectiveness analysis

Decisions about health interventions are often made using limited evidence. Mathematical models used to inform such decisions often include uncertainty analysis to account for the effect of uncertainty in the current evidence base on decision-relevant quantities. However, current uncertainty quantification methodologies, including probabilistic sensitivity analysis (PSA), require modelers to specify a precise probability distribution to represent the uncertainty of a model parameter. This study introduces a novel approach for propagating parameter uncertainty, probability bounds analysis (PBA), where the uncertainty about the unknown probability distribution of a model parameter is expressed in terms of an interval bounded by lower and upper bounds on the unknown cumulative distribution function (p-box) and without assuming a particular form of the distribution function. We give the formulas of the p-boxes for common situations (given combinations of data on minimum, maximum, median, mean, or standard deviation), describe an approach to propagate p-boxes into a black-box mathematical model, and introduce an approach for decision-making based on the results of PBA. We demonstrate the characteristics and utility of PBA versus PSA using two case studies. In sum, this study provides modelers with practical tools to conduct parameter uncertainty quantification given the constraints of available data and with the fewest assumptions.

==> word_count.tex <==
\begin{document}

\begin{frontmatter}
\maketitle

\begin{abstract}
Decisions about medical devices in the early phase of their lifecycles are often made using limited evidence. Mathematical models used to inform such decisions often include probabilistic sensitivity analysis (PSA) to account for the effect of uncertainty in the current evidence-base on decisional-relevant quantities. However, current methodologies for conducting PSA require modelers to specify a precise probability distribution to represent the uncertainty of a model parameter. This study introduces a novel approach for propagating parameter uncertainty, a probability bounds analysis (PBA), where the uncertainty about the probability distribution of a model parameter is expressed in terms of lower and upper bounds on the cumulative distribution function (p-box) and without assuming a particular form of the distribution function. We show the derivation of the p-boxes for common situations (given combinations of data on minimum, maximum, median, mean, or standard deviations), describe an algorithm to propagate p-boxes into a decision model, and introduce an approach for decision-making based on the results of a PBA. Then, we demonstrate two applications of PBA in detail. In sum, this study will provide modelers with tools to inform decision-making given constraints of available data with the fewest number of assumptions.
% Please include a maximum of seven keywords
\keywords{Cost-effectiveness analysis, decision-analytic modeling, parameter uncertainty, uncertainty quantification}
\end{abstract}
\end{frontmatter}

\section{Introduction}
The importance of explicitly accounting for incomplete knowledge about model parameters (e.g., in terms of uncertainty) and propagating its effect through the decisional process is underscored in numerous guidance documents in health, including, but not limited to, the guidelines by the International Society for Pharmacoeconomics and Outcomes Research (ISPOR)-Society for Medical Decision Making (SMDM),\cite{briggs2012model} the Agency for Healthcare Research and Quality (AHRQ),\cite{dahabreh2016recommendations} the 2nd panel for Cost-Effectiveness Analysis (CEA) in Health and Medicine,\cite{sanders2016recommendations} and beyond.\cite{national2012assessing}
At its most basic characterization, parameter uncertainty means that we do not know the exact value of a parameter as several different (potentially uncountable) values may be possible.
In most situations, the only information we have about a parameter is that it belongs to an interval bounded by a lower bound and an upper bound.
In addition to knowing the interval, we may have some information about the relative plausibility of different values of $\theta$ in the interval.
%we need to assert which values in the interval are more probable than other values. 
In situations where we have data or previous knowledge about a parameter, we can leverage standard statistical techniques to represent uncertainty in the form of a probability distribution.
%or through sufficient summary statistics.
However, when data is limited, we may have only partial information about the probability distribution. 
In some cases, we may know the measures of central tendency (mean or median); while, in more extreme cases, only the minimum and maximum values are known to the researchers.
To handle such data sparsity situations, it is necessary to have an approach for quantifying parameter uncertainty using the fewest number of assumptions.
\\ \\
Despite the emphasis on its importance, the best-practice in decision-analytic modeling\cite{briggs2012model} recommends only two analytical tools for evaluating the effect of incomplete knowledge of model parameters on decisional-relevant outcomes despite the wealth of available methods in engineering literature.
First, the best practice prescribes a set of default distributions, that are mainly driven by the consideration of the parameter's support.
For example, a beta distribution is used for characterizing uncertainty of a parameter with a support $[0,1]$.
As a result, modelers tend to rely on "off-the-shelf" probability distributions to portray uncertainty "realistically over the theoretical range of the parameter."\cite{briggs2012model}
% However, despite cautioning against the use of "convenient-to-fit, but implausible, distributions,"
The use of such default distributions is in fact a matter of convenience because there is no sure way to verify that our choice of distribution and its parameters is indeed valid.
Furthermore, forcing the modelers to commit to a particular distribution implicitly assumes that the modelers have more information (e.g., knowing the shape of a distribution) than they actually possess and that the uncertainty is known and quantifiable by a probability distribution.
Secondly, the best practice proposes the use of expert knowledge elicitation\cite{ohagan2006uncertain} if prior data is not available.
However, such solution also hinges on a rather unverifiable assumption: the precise form of the probability distribution.
The lack of such methodological guidance is due to the lack of a formal comprehensive characterization of different levels of parameter uncertainty.
\\ \\
% An approach that maximizes the use of existing (limited) information, albeit, with the fewest assumptions is desirable.
% Our approach of representing the uncertainty of a parameter does not require the specification of a probability distribution type and requires data as minimal as the range.
% The common approach to model our incomplete knowledge about the values of some parameters is to assume those parameters follow a uniform distribution.
% In fact, this most common criterion for choosing initial probabilities distribution is related to the \textit{Principle of Insufficient Reason} coined by Laplace~\cite{laplace1812marquis} more than two centuries ago (also known as the Principle of Indifference) ~\cite{keynes2013treatise}).
% However, such an assumption is not as harmless as one may perceive.
% The criticisms of the principle was voiced as early as 1812 by the British economist, Keynes. ~\cite{keynes2013treatise}
% However, it is assumed here that such probability distributions are not known, and “forcing” a distribution may do more harm to the decision-making process than good.
%
 %the use of "off-the-shelf" probability distribution
 %
% Taleb\cite{taleb2007black} warned that parametric uncertainties and estimation errors in probability distributions can result
% in adverse effects in the understanding of extreme events. 
% A distribution-driven approach can overemphasize the mean value of the distribution and ignore important information in its tails.
% The lack of such methodological guidance is due to the lack of a formal comprehensive characterization of different levels of parameter uncertainty.
An ideal approach to parameter uncertainty characterization is the one that requires minimal assumptions .
Specifically, such approach should require only information on statistics that are typically accessible to practitioners, such as mean, median, quantiles, minimum, and maximum.
Additionally, the ideal method does not require information on or assumption about the form of a probability distribution.
% and the dependencies between the model parameters.
% Empirical information about dependencies among variables in an assessment is often sparse. 
% In multivariate problems, it is commonly not practical to specify the entire variance-covariance matrix (Cooke 1997), much less the full multidimensional character of the dependence among the variables.
% Lastly, the optimal strategy must be selected not only according to their predicted outcomes, but also according to the immunity of those outcomes to errors in the knowledge underlying the predictions, and according to the opportunities inherent in the uncertainty.
Probability bounds analysis, a combination of interval analyses and probability theory, is one such method.\cite{ferson2015constructing}
In a probability bounds analysis, the uncertainty about the probability distribution for each input variable is expressed in terms of interval bounds on the cumulative distribution function (CDF). 
These CDF bounds form a ‘p-box’ for each input variable. 
These information are sufficient for circumscribing the distribution of a random variable given some limited information about it.
We focus on \textit{free p-boxes} that is a generalization of parametric p-boxes, which are defined as a distribution the parameters of which are modelled by intervals.
\\ \\
The goal of this paper is to introduce a method for characterizing and propagating parameter uncertainty in situations where knowledge about the parameter is limited and a probability distribution can not be specified precisely or the practitioners are not willing to commit to a particular form.
First, I explicate the concept of parameter uncertainty quantification in which I briefly review existing approaches in the decision analysis literature.
Then, I formally introduce the concept of probability bounds.
Secondly, I describe the problem of propagating parameter uncertainty into a mathematical model.
Then, I outline an algorithm for conducting probability bound analyses and demonstrate its application using a clinical decision-making problem.
Lastly, I conclude with a discussion on the limitations and directions for future research.
%\section{Characterizing parameter uncertainty}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{[THERE MAY BE A BRIEF SECTION ON THE NOTION OF PARAMETER UNCERTAINTY]}
\section{Probability box}
\subsection{Definition}
Suppose that the (imperfect) knowledge about a continuous random variable ($\theta$) can be characterized by its cumulative distribution function (CDF), $F(\theta)$, which is a monotonically increasing function from $\mathbb{R}$ onto $[0,1]$, zero at negative infinity, and one at positive infinity.
A probability box or \textit{p-box} consists of a pair of CDFs that circumscribe an imprecisely known $F(\theta)$.[REF]
Formally, a p-box of a continuous random variable $\theta$ with an unknown CDF $F(\theta)$ is a pair of bounding functions, i.e., a lower-bounding function (LBF) $\uF$ and an upper-bounding function (UBF) $\lF$, or $\mathcal{P}_{\mathcal{D}}=\{\lF,\uF\}$, where $\mathcal{D}$ denotes the type of available data.
The UBF and LBF have the following properties:
\begin{enumerate}
    \item $\lF$ and $\uF$ are CDFs
    \item $\lF \le F(\theta) \le \uF$ for $\forall \theta$ in the support of $F(\theta)$
    \item $\lF$ and $\uF$ form the "tightest" p-box
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Formulas for different $\mathcal{D}$}
We consider commons situations of data availability where a modeler can identify and specify a combination of different summary statistics of $\theta$.
The derivation of the formulas can be found in the Appendix \ref{app:pbox_derivation}.
The first situation involves knowing the smallest (minimum) and largest (maximum) values of a parameter.
For some parameters, one can infer the range from theoretical limits, such as zero to one for probability or utility parameters. 
In some cases, a modeler may ask domain experts to specify a range from their specific or general knowledge about the quantity in question.
In both cases, the task will set $\ltt$ and $\utt$ such that $\theta \in [\lt , \ut] \define I_\theta$.
The $\mathcal{P}_{I_\theta}$ is given by:
\begin{align}
    \lF = \begin{cases}
     0 \quad &\mbox{ for } \quad \theta < \ut \\
    1 \quad &\mbox{ for } \quad \ut \le \theta\\
    \end{cases}
\end{align}
for LBF, and, 
\begin{align}
    \uF = \begin{cases}
     0 \quad &\mbox{ for } \quad \theta < \lt \\
    1 \quad &\mbox{ for } \quad \lt \le \theta\\
    \end{cases}
\end{align}
for UBF.
%\subsubsection{Median, min, and max}
\\ \\
If, in addition to knowing $I_\theta$, the median ($m$) of the parameter is also known, the p-box can be tighter.
The $\mathcal{P}_{I_\theta,m}$ is given by:
\begin{align}\label{eq: pbox_median_LBF}
    \lF = \begin{cases}
     0 \quad &\mbox{ for } \quad \theta < m \\
    0.5 \quad &\mbox{ for } \quad m \le \theta < \utt\\
        1 \quad &\mbox{ for } \quad \utt \le \utt\\
    \end{cases}
\end{align}
for LBF, and, 
\begin{align}
    \uF = \begin{cases}
     0 \quad &\mbox{ for } \quad \theta < \ltt \\
    0.5 \quad &\mbox{ for } \quad \ltt \le \theta < m\\
        1 \quad &\mbox{ for } \quad m \le \utt\\
    \end{cases}
\end{align}
for UBF. \\ \\
%\subsubsection{Mean, min, and max}
If, in addition to knowing $I_\theta$, the mean ($\mu=E[\theta]$) is also known , the p-box can be tighter. 
The $\mathcal{P}_{I_\theta,\mu}$ is given by:
\begin{align} \label{eq:pbox_mean}
    \lF = \begin{cases}
     0 \quad &\mbox{ for } \quad \theta < \mu \\
    \frac{\theta-\mu}{\theta-\ltt} \quad &\mbox{ for } \quad \my \le \theta\\
    \end{cases}
\end{align}
for LBF, and, 
\begin{align}
    \uF = \begin{cases}
     \frac{\utt-\mu}{\utt-\theta} \quad &\mbox{ for } \quad \theta < \ltt \\
    1 \quad &\mbox{ for } \quad \ltt \le \theta\\
    \end{cases}
\end{align}
%\subsubsection{Mean, standard deviation min, and max}
If, in addition to the mean, we have data on the standard deviation ($\sigma$), then the $\mathcal{P}_{I_\theta,\mu,\sigma}$ is given by:
\begin{align} \label{eq:pbox_std_lower}
    \lF = \begin{cases}
     0 \quad &\mbox{ for } \quad \ltt \le \theta \le \xi_1 \\
    \frac{\sigma^2+(b-\mu)(\theta-\mu}{(\utt-\ltt)(\theta-\ltt)} \quad &\mbox{ for } \quad \xi_1 \le \theta <\xi_2\\
        \frac{(\theta-\mu)^2}{(\theta-\mu)^2 + \sigma^2} \quad &\mbox{ for } \quad \xi_2 \le \theta \le \utt\\
    \end{cases}
\end{align}
for LBF, and, 
\begin{align} \label{eq:pbox_std_upper}
    \uF = \begin{cases}
      \frac{\sigma^2}{(\mu-\theta)^2+\sigma^2}  \quad &\mbox{ for } \quad \ltt \le \theta \le \xi_1 \\
    \frac{(\utt-\mu)(\utt-\ltt+\mu-\theta) - \sigma^2}{(\utt-\ltt)(\ut-\theta)} \quad &\mbox{ for } \quad \xi_1 <= \theta <\xi_2\\
       1 \quad &\mbox{ for } \quad \xi_2 \le \theta \le \utt\\
    \end{cases}
\end{align}
for UBF, where $\xi_1 = \mu - \frac{\sigma^2}{b-\mu}$ and $\xi_2 = \mu + \frac{\sigma^2}{\mu-a}$.
\\ \\
We can derive further cases by intersecting the p-box of each $\mathcal{D}$ described above (termed as primitive p-boxes) by "tracing" the minimum (or maximum) of the intersection of the corresponding UBFs (or LBFs).
More formally, for each $\mathcal{D}_{d}$ (where $d$ indexes each combination of data), the LBF and UBF are given by:
\begin{align}
    \lF=\max \lF_{\mathcal{D}_{d_1}} \lF_{\mathcal{D}_{d_2}} \ldots \lF_{\mathcal{D}_{d_n}}
\end{align}
and
\begin{align}
    \uF=\min \uF_{\mathcal{D}_{d_1}} \uF_{\mathcal{D}_{d_2}} \ldots \uF_{\mathcal{D}_{d_n}},
\end{align}
respectively ($d_i$ indexes the primitive p-boxes included in a particular $d$.
Figure \ref{fig:pbox_input} illustrates p-boxes associated with different $\mathcal{D}$.
\begin{figure}[bt]
\centering
\includegraphics[width=14cm]{multi_latest.png}
\caption{P-boxes with different $\mathcal{D}$ and a normal cumulative density function. Note: All $\mathcal{D}$s include minimum (min) and maximum (max). CDF: cumulative distribution function, SD: standard deviation.}
\label{fig:pbox_input}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Uncertainty propagation}
Let $\mathcal{M}$ denote a mathematical model (e.g., a cost-effectiveness model\cite{sanders2016recommendations} or a decision-analytic model\cite{iskandar2018theoretical}) that maps a set of $k$ inputs $\bu{\theta}$ to a set of quantities of interest $\bu{Y}$, i.e.,  $\mathcal{M}: \bu{\theta} \rightarrow \bu{Y}$.
We treat $\mathcal{M}$ as a black-box model, i.e., only $\bu{\theta}$ and the corresponding $\bu{Y}$, after "running" $\mathcal{M}$ at $\bu{\theta}$, are accessible. 
Our uncertainty about each parameter in $\bu{\theta}$ may vary according to the extent of what is known.
In principle, each $\theta_i$, based on the characterization of its uncertainty, falls into of the following subsets of $\bu{\theta}$: (1) $\bu{\theta}_f$ for fixed parameters, (2) $\bu{\theta}_c$ for parameters known up to their CDFs , and (3) $\bu{\theta}_b$ for parameters with severe uncertainties.
The propagation of uncertainty of $\bu{\theta}_c$ is straightforward, e.g., by using Monte Carlo sampling.
Here, we first focus on describing how to propagate p-boxes in the context of $\bu{\theta}_c$. 
Then, we outline how to propagate uncertainties from both $\bu{\theta}_c$ and  $\bu{\theta}_b$ into $\mathcal{M}$.
% An uncertainty propagation of all p-boxes is, in principle, the estimation of the lower and upper bounds of the cdf, the p-box, of $\bu{Y}$.
% To propagate a p-box, one could use full-factorial design (FFD) or random sampling approaches.
\subsection{Propagating p-boxes}
To propagate uncertainty of the set $\bu{\theta}_b$ , first, for each $\theta_i \in \bu{\theta}_b$, we specify its p-box given $D_i$.
To build intuitions about how the uncertainty propagation for p-box parameters works, we use a full-factorial-design approach, i.e., slicing algorithm,\cite{zhang2010interval} and follow the steps in \cite{schobi2017uncertainty}.
The algorithm discretizes a p-box into intervals with their associated probability masses.
For each $\theta_i$, the interval $[0,1]$ is divided into $n_{\theta_i}$ subintervals with its corresponding probability mass $p_j$ ($j \in \{1, 2, \ldots,n_{\theta_i}\}$ such that $\sum\limits_{j=1}^{n_{\theta_i}} m_j = 1$.
For the $j$-th subinterval, we identify their boundary points: $\lc_i^j$ and $\uc_i^j$.
Given each pair of boundary points, we calculate the boundary points in the $\theta$ domain by using the inverse p-box functions (or quantile functions):
\begin{align}
    \ltt_i^{j} = \uF^{-1}\left(\lc_i^j\right), \quad \quad \utt_i^{j} = \lF^{-1}\left(\uc_i^j\right)
\end{align}
These quantile functions are derived from their corresponding LBF and UBF.
The interval $[\lt^{j},\ut^{j}]$ and its associated $m_j$ form the p-box of $\theta_i$.
\\ \\
The number of p-boxes depends on $n_{\theta_i}$ subintervals for each $\theta_i$.
We denote $\mathcal{K}$ as the set of multi-indices where each multi-index corresponds to a particular combination of sub-intervals across $\theta$s:
\begin{align}\label{eq:K}
    \mathcal{K}={\bu{k}=(k_1, k_2, \ldots, k_n)}, \quad \quad k_i \in [1, \ldots, n_{\theta_i}]
\end{align}
where $n$ is the number of parameters in $\bu{\theta}_p$.
For each $\bu{k} \in \mathcal{K} $, we denote $\mathcal{H}_\bu{k}$ as a hyperrectangle (i.e., a Cartesian product of intervals) which is given by:
\begin{align}\label{eq:H_k}
    \mathcal{H}_{\bu{k}} = \left[\ltt_1^{k_1},\utt_1^{k_1}\right] x \left[\ltt_2^{k_2},\utt_1^{k_2} \right] x \ldots \left[\ltt_n^{k_n},\utt_1^{k_n} \right]
\end{align}
For each $\mathcal{H}_{\bu{k}}$ we calculate its probability mass as follows:
\begin{align}
    P(\mathcal{H}_{\bu{k}}) = m_{k_1}  m_{k_2} \ldots  m_{k_n}
\end{align}
For each $\mathcal{H}_{\bu{k}}$, we associate two optimization problems whose solutions provide the bounds on a quantity of interest $\bu{Y}$:
\begin{align}
    \lY^{\bu{k}} = \min_{\bu{\theta}_b} \mathcal{M}(\bu{\theta}_b), \quad \quad \uY^{\bu{k}} = \max_{\bu{\theta}_b} \mathcal{M}(\bu{\theta}_b)
\end{align}
for fixed values of $\theta$s in $\bu{\theta}_f$ and  $\bu{\theta}_c$.
The existence of a maximum and a minimum is guaranteed by the Weierstrass Extreme Value Theorem\cite{rudin1964principles} since, in decision-analytic modeling, the model $\mathcal{M}$ is typically smooth and $\mathcal{H}_{\bu{k}}$ is closed and bounded (compact).
The p-box of $Y$ is therefore characterized by $\left[\lY^{\bu{k}},\uY^{\bu{k}}\right]$ and its corresponding probability mass $P(\mathcal{H}_{\bu{k}})$.
The empirical p-box of $Y$ can be calculated as:
\begin{align}\label{eq:cdf_Y}
 \lF(Y)=\sum\limits_{i=1}^{|\mathcal{K}|}  P(\mathcal{H}_{\bu{k}_i}) \mathcal{I}_{\lY_i \le Y}   , \quad \quad \uF(Y)=\sum\limits_{i=1}^{|\mathcal{K}|}  P(\mathcal{H}_{\bu{k}_i}) \mathcal{I}_{\uY_i \le Y} 
\end{align}
\subsection{Propagating p-boxes and other parameters} \label{sec:propagate_theta_c}
In some cases, practitioners may have access to information that is sufficient for specifying probability distributions of parameters ($\bu{\theta}_c$).
To propagate uncertainty from both sets $\bu{\theta}_c$ and $\bu{\theta}_b$ into $\mathcal{M}$, we proceed in two steps.
First, since the uncertainty of each parameter in $\bu{\theta}_c$ can be characterized by a precise probability function, the uncertainty propagation reduces to Monte Carlo approach,\cite{cullen1999probabilistic} a repeated sampling from a joint distribution of parameters in $\bu{\theta}_c$ (if their dependencies are known).
Let $f(\bu{\theta}_c)$ be the joint distribution.
Repeated sampling from $f(\bu{\theta}_c)$ will generate a sequence of samples of $\bu{\theta}_c$: $\bu{\theta}_c^{1}, \bu{\theta}_c^{2}, \ldots, \bu{\theta}_c^{N}$, where $N$ is the total number of samples. 
Second, for each sample  $\bu{\theta}_c^{l}$ and each $\mathcal{H}_k$ (Equations \ref{eq:K} and \ref{eq:H_k}), we solve:
\begin{align}
    \lY^{\bu{k},l} = \min_{\bu{\theta}_c} \mathcal{M}(\bu{\theta}_b,\bu{\theta}_f,\bu{\theta}_c^l), \quad \quad \uY^{\bu{k},l} = \max_{\bu{\theta}_c} \mathcal{M}(\bu{\theta}_b,\bu{\theta}_f,\bu{\theta}_c^l)
\end{align}
and derive $\lF^l(Y)$ and $\uF^l(Y)$ using Equation \ref{eq:cdf_Y}.
The p-box of $Y$ is then calculated by averaging over the $N$ samples:
\begin{align}
    \widehat{\lF}(Y)=\sum\limits_{l=1}^{N}=\lF^l(Y), \qquad \widehat{\uF}(Y)=\sum\limits_{l=1}^{N}=\uF^l(Y)
\end{align}
\section{Case study: $4$-state Markov model}
We conduct a case study to demonstrate: (1) the effect of having more data on the tightness of the bound on a QoI , and (2) how to conduct a PBA.
The model is coded in R \cite{R2019} as open-source programs have emerged as the lingua franca for practitioners in decision-analytic modeling. \cite{DARTH2019,jalal2017overview}
The code is available under a GNU GPL license and can be found at https://github.com/rowaniskandar/PBA.
\subsection{Model description}
We consider a generic four-state stochastic cohort model with the following health states $\mathbb{S}=\{S_1, S_2, S_3, S_4\}$ (Figure \ref{fig:4statesdiagram_2}), where $S_4$ is an absorbing state.
We assume that the transition rate from $S_1$ to $S_2$ is precisely known ($c_{12}=0.05$).
For the rates for transitions $S_1 \rightarrow S_3$, $S_2 \rightarrow S_3$, and $S_3 \rightarrow S_4$, we use gamma distributions with parameters $\{\mu=0.01,\sigma=0.0033\}$, $\{\mu=0.1,\sigma=0.033\}$, and $\{\mu=1,\sigma=0.33\}$ respectively. 
The uncertainty around rates of transitions $S_1 \rightarrow S_4$ and $S_2 \rightarrow S_4$ are modeled using p-boxes with $\mathcal{D}=\{\lt=0,\ut=10,\mu=0.001,\sigma=0.000333\}$ and $\mathcal{D}=\{\lt=0,\ut=10,\mu=0.05,\sigma=0.0167\}$, respectively.
We also conduct an analysis where we assume that the rates of transitions $S_1 \rightarrow S_4$ and $S_2 \rightarrow S_4$ follow a gamma distribution, as a comparison to the p-box approach.
For a QoI, we calculate the expected residence time in states other than $S_4$ or "life expectancy" (Figure \ref{fig:pbox_QoI}). 
\begin{figure}[bt]
\centering
\includegraphics[width=9cm]{4states_diagram2.png}
\caption{A state-transition model diagram  used in case study 1}
\label{fig:4statesdiagram_2}
\end{figure}
\begin{figure}[bt]
\centering
\includegraphics[width=10cm]{pbox_QoI.png}
\caption{Uncertainty around QoI of $4$-state model using p-boxes and precise CDFs for some parameters vs. using precise CDFs for all parameters. CDF: cumulative distribution function, LBF: lower bounding function, UBF: upper bounding function.}
\label{fig:pbox_QoI}
\end{figure}
\subsection{Model analyses}
% We calculate the average number of individuals,\cite{iskandar2018theoretical} with an initial condition: everyone start in $S_1$, i.e. $N_1(0)=1000$, for a 50-years duration.
% \subsection{Case study: Border screening for deadly virus [WILL BE REMOVED]}
% To demonstrate the utility and application of the PBA, we consider a decisional problem where public health officials are tasked with screening for a life-threatening transmissible viral disease among people arriving at a country's entry point (e.g., airport or land border).
% Our example closely follows that of Troffaes and Gosling \cite{troffaes2012robust} and adopts the same notations.
% Below we formally specify the decisional problem.
% \\ \\
% Let $n$ be the number of people entering the area; among those, $d$ people are unknowingly infected with the virus.
% Officials can randomly test $m$ ($<n$) people.
% A choice of a particular value of $m$, hence, constitutes a strategy
% The test is assumed to be imperfect with sensitivity $p$ and specificity $q$, and it costs $c$ per test.
% If an infected person entered the area undetected (i.e., a false negative case or not selected for testing), then the area will incur a (catastrophic) cost of $a(d)$.
% If $z$ ($1 \le z \le m$) people were diagnosed with the virus, everyone ($n$) will be quarantined; thereby incurring a "cost" of $t(n)$.
% The expected loss of the screening strategy is given by
% \begin{align}
%     L(m,d,p,q,c,a,t)=c(m) + t(n) Pr[T\vert d] + a(d) Pr[T^c\vert d]
% \end{align}
% where $T$ denotes the event that at least one person ($z\ge 1$) is diagnosed among $m$ samples and $T^c$ denotes its complement ($z=0$).
% The probability of exactly $z$ diseased people among $m$ tested people follows a hypergeometric distribution (due to sampling without replacement) and is given by $Pr[z\vert d]=\frac{\binom{d}{z}\binom{n-d}{m-z}}{\binom{n}{m}}$.
% The probability of non-quarantine given $d$ is estimated by:
% \begin{align} \label{eq:eq_prob_d_r}
%     \sum\limits_{z=0}^{d} (1-p)^z q^{m-z} \frac{\binom{d}{z}\binom{n-d}{m-z}}{\binom{n}{m}}
% \end{align}
% To model the number of infected individuals $d$, we use a binomial model where we assume that each individual can be infected with a probability $r$ and independence among individuals (i.e., an individual's infection status does not affect the others' risk of infection).
% Under these assumptions, the probability of having $d$ infected individuals out of $n$ is given by $Pr[d \vert r]=\binom{n}{d}r^d(1-r)^{n-d}$.
% The expected loss across possible values of $d$, given $r$, is equal to:
% \begin{align}
%     E[L(m,.,p,q,c,a,t)\vert r] = \sum\limits_{d=0}^{n} L(m,d,p,q,c,a,t) Pr[d \vert r]
% \end{align}
% By fixing some quantities and focusing on a key decision parameter, i.e., the number of people to be tested ($m$) and one input with deep uncertainty, i.e., the probability of infection ($r$), we have
% \begin{align}
%     L(m \vert r)= \sum\limits_{d=0}^{n} L(m,d,p,q,c,a,t) Pr[d \vert r]
% \end{align}
% We assume that the overall mean cost was USD 6827 per treated infection episode.\cite{li2020treatment}.
% \\ \\
% We emphasize that the example is intended for demonstrating the value of PBA, but not for providing qualitative conclusions about the decisional problem.
% Appendix X gives details on the derivation of the above equations.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
This study introduces a probability bound analysis for quantifying the effect of parameter uncertainty on model outcomes. 
The novel uncertainty quantification method represents a general framework to represent imprecisely specified distributions, i.e., without assuming a particular form of the probability distribution.
In a PBA, parameter uncertainties are characterized by p-boxes that provide the maximum area of uncertainty (tightest bounds) containing the unknown distribution function, given knowledge about summary statistics.
To assist practitioners in the fields of decision-analytic modeling and economic evaluation, we provide p-box formulas for most common situations of data availability.
Then, we demonstrate how to propagate p-boxes into a black-box model where the uncertainty of the model parameters are characterized by a combination of p-boxes and parametric distribution functions using a case study.
The novel approach allows practitioners to conduct probabilistic assessment even when extremely little reliable empirical information is available about the distributions of model parameters.
In a way, a p-box is a generalization of the standard approach for representing parameter uncertainty using a single CDF, i.e., if the lower and upper bounds of the CDF coincide for every element in the support, then the p-box degenerates to one CDF.
\\ \\
One decisional-relevant information from the results of a PBA is likely to be the bounds on the tail probabilities of a QoI, particularly, when the QoI represents a negative outcome (or a catastrophic event).\cite{tucker2003probability}
The p-box of a QoI essentially provides information that a QoI will not be smaller (or larger) than a minimum (or maximum), which can be identified by the infimum (supremum) of the support of the UBF (LBF). 
Futhermore, assuming a particular distribution for a parameter may potentially lead to an underestimation of the probability of observing extreme values of QoI (Figure \ref{fig:pbox_QoI}).
\\ \\
The reliance on using "off-the-shelf" probability distributions for characterizing uncertainty about model parameters can be mitigated by using expert opinion.\cite{garthwaite2005statistical}
However, assessing probabilities from experts can be difficult and are not free from biases including representativeness, availability, and anchoring and adjustment that can lead to incorrect and misjudged probabilities.\cite{bedford2001probabilistic,tversky1971belief}
Using probability distribution may also assume more information about uncertainty than is warranted. 
These errors in estimating probabilities can lead to overconfidence and a failure to protect against highly consequential risks.\cite{taleb2007black}
If the probability distribution is not known, it could be assessed via expert judgment. 
However, probability distributions derived from
expert elicitation can suffer from a number of errors.\cite{fischhoff1977knowing,lin2008study}
In situations where best-case/worst-case results are the basis for decision making, the analytical interval approach is preferred to assuming a distribution (e.g., uniform) and performing a simulation, particularly when that distribution may not correctly describe the parameters.
\\ \\
PBA is computationally intensive for the following reasons. 
First, an implementation of a PBA requires an optimization step over the p-box.
In this study, we use a full factorial design that transforms the problem of propagating a p-box into a propagation of a large number of intervals.
The higher the required level of accuracy is, the higher number of intervals $n_{\theta_i}$ is needed.
Furthermore, an increase in the number of p-box parameters will lead to a higher-dimensional optimization problem.
Second, the computational burden is further exacerbated if a black-box model ($\mathcal{M}$) is "expensive" to evaluate, given a set of $\theta$.
Thirdly, if, in addition to p-box parameters, some parameters are characterized by their CDFs, the optimization step is embedded in a Monte Carlo sampling loop (Section \ref{sec:propagate_theta_c}); thereby increasing the number of optimizations by a factor of $N$ (the total number of Monte Carlo samples).
To mitigate the computational burden, users of PBA may opt to use more conservative p-box propagation approaches,\cite{schobi2017uncertainty}, more efficient optimization methods\cite{deng2013improved}, and fast-to-evaluate approximations of the original model or meta-models.\cite{ellis2020active}
Nevertheless, we expect a higher computational burden since a PBA imposes less restrictions (i.e., we don't assume a functional form), leading to a larger region of uncertainty over which a model needs to be evaluated.
% In particular, the probability of extreme values is seen to be potentially much greater than would be predicted by a one-dimensional Monte Carlo analysis, although it is not possible to conclude that they necessarily will be. 
% The uncertainty in these probabilities is a direct consequence of the uncertainty in the input distributions.
%usefulness of pbox
%fat tail (low prob, high consequences)
%bounds refer to different choice
%worse/best case decision-making 
\\ \\
A p-box is closely connected to Dempster-Shafer’s theory of evidence.\cite{dempster2008upper,shafer1976mathematical,ferson2015constructing}
The LBF and UBF are interpreted as belief and plausibility measures for the event $\theta$ taking values than a particular value $\{\theta \le x\}$. 
In Dempster-Shafer’s theory, the belief function describes the minimum amount of probability that must be associated with the event; whereas the plausibility function describes the maximum amount of probability that might be associated to the same event.
The PBA framework is also related to Bayesian sensitivity analysis (or robust Bayesian analysis).\cite{berger1990robust}
In this approach, an analyst’s uncertainty about which prior distribution and likelihood function should be used is characterized by entire classes of prior distributions and likelihood functions. 
The analysis proceeds by studying the variety of outcomes for each possible combination of prior distribution and likelihood function. 
Another distribution-free approach is the Chebyshev inequality\cite{saw1984chebyshev} that can be used to compute bounds on the CDF of a random variable, given the mean and standard deviation of the random variable.
However, the inequality cannot produce a tighter bound even if we have more data (e.g., median).
Kolmogorov-Smirnov (KS) confidence limits\cite{saw1984chebyshev} also provide distribution-free bounds to an empirical CDF. 
The calculation of KS limits require, however, requires access to sample data.
% %K-S limits
% How should we account for sampling uncertainty that arises from measuring only a portion of the population? 
% It would seem reasonable to inflate the uncertainty about the empirical histograms in some way. 
% The sampling theory for probability bounds analysis and Dempster-Shafer theory needs more development, but one strategy suggests itself. 
%limitation of current approaches
% One should be wary of equating knowing the moments (mean and variance) to knowing a probability distribution.
% Mathematically, the distribution of a random variable may fail to have a mean or variance (e.g., Cauchy distribution).
\\ \\
Our study has limitations in the following context.
First, we assume independence among the model parameters.
One potential approach for modeling dependencies among parameters is to use a copula to represent the joint uncertainty of all parameters.\cite{joe1997multivariate}
A copula approach factors the joint CDF into a product of independent marginal CDFs and a copula that capture the dependencies.
In this formulation of bounds using a joint CDF, the overall bound is a function of the bounds on CDFs for some parameters represented by their p-boxes and the bounds of the copula.
The potentially promising approach using copula warrants further study and is, however, beyond the scope of our study.
Secondly, our study does not address the question of when one should consider using p-box vs. assuming a particular CDF to characterize uncertainty.
Instead of being prescriptive, we defer such decisions to the analysts because the level of uncertainty at which a p-box is the preferred approach is problem-dependent.
For example, a parameter may be highly uncertain due to the lack of empirical data and/or previous knowledge and, at the same time, non-influential, i.e., the QoI is not sensitive to variations in the parameter values.
Thirdly, we provide a rudimentary treatment on how to decision-making  
In situations where best-case/worst-case results are the basis for decision making, the analytical interval approach is preferred to assuming a distribution (e.g., uniform) and performing a simulation, particularly when that distribution may not correctly describe the parameters.
A more comprehensive treatment of decision-making based on interval values or bounds on probability distributions is needed and should be a focus of future studies on uncertainty quantification in decision-analytic modeling and cost-effectiveness analysis.
\section{Concluding remarks}
The proposed study addresses limitations in current methodologies for characterizing uncertainty in parameter estimates used to inform decision-making.
The novel approach provides a way to honestly characterize the uncertainty in the model parameters' distributions used in decision-analytic modeling and cost-effectiveness analysis studies.
